Evolving Mobile Cloud Gaming with 5G Standalone Network Telemetry

Mobile cloud gaming places the simultaneous demands of high capacity and low latency on the wireless network, demands that Private and Metropolitan-Area Standalone 5G networks are poised to meet. However, lacking introspection into the 5G Radio Access Network (RAN), cloud gaming servers are ill-poised to cope with the vagaries of the wireless last hop to a mobile client, while 5G network operators run mostly closed networks, limiting their potential for co-design with the wider internet and user applications. This paper presents Telesa, a passive, incrementally-deployable, and independently-deployable Standalone 5G network telemetry system that streams fine-grained RAN capacity, latency, and retransmission information to application servers to enable better millisecond scale, application-level decisions on offered load and bit rate adaptation than end-to-end latency measurements or end-to-end packet losses currently permit. We design, implement, and evaluate a Telesa telemetry-enhanced game streaming platform, demonstrating exact congestion-control that can better adapt game video bitrate while simultaneously controlling end-to-end latency, thus maximizing game quality of experience. Our experimental evaluation on a production 5G Standalone network demonstrates a 178-249% Quality of Experience improvement versus two state-of-the-art cloud gaming applications.

==> sections/Attic.tex <==

%In 4G, PDCCH occupies the whole downlink channel and Downlink Control Information (DCI) is transferred plain text, so one can decode the DCI and then infer user's RNTI.
%The Physical Downlink Control Channel (PDCCH) of 5G only uses part of the cell's channel, which is called Control Resource Set (CORESET) and is scrambled by Radio Network Temporary Identifier (RNTI)~\cite{project_3gpp_2023-3}.
%In our work, we overcome this obstacle by decoding some of base station's Radio Resource Control (RRC) messages , including master information block (MIB) and system information block (SIB) 1, as well as user equipment (UE)'s intial random access procedure (RACH), during which the base station provides all the parameters we need for decoding the physical channel and UE's C-RNTI.

% \subsubsection{Term Definitions} 

% We list the terms and their definition that we use in the following sections here as a reference.
% %
% Table~\ref{tab:physical_channel} shows the definition of physical channels in 5G RAN, and one thing needs mentioning is that RACH is the physical channel for UE's intial random access, and it's common to use RACH process to refer to UE's random access procedure, \textit{e.g.} the messages exchange from MSG 1 to MSG 4. 
% %
% Table~\ref{tab:rrc} provides the definition for RRC messages and DCI, and Table~\ref{tab:rnti} provides the definition for RNTIs. ({\color{red} We should put the content in these tables into the sentences where these terms show up the first time, I'll change it into this way.})

% \begin{table}[]
% \centering
% \begin{tiny}
% \begin{tabular}{l|l}
% \hline
% \multicolumn{1}{c|}{Terms}                                                           & \multicolumn{1}{c}{Definition}                                                                                                                                                               \\ \hline
% \begin{tabular}[c]{@{}l@{}}Physical Broadcast \\ Channel (PBCH)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}PBCH serves as the primary channel through which \\ a base station transmits master information block \\ and synchronization signals and to UEs.\end{tabular}     \\ \hline
% \begin{tabular}[c]{@{}l@{}}Physical Downlink \\ Control Channel (PDCCH)\end{tabular} & \begin{tabular}[c]{@{}l@{}}PDCCH is the physical channel that carries \\ downlink control information.\end{tabular}                                                                          \\ \hline
% \begin{tabular}[c]{@{}l@{}}Control Resource \\ Set (CORESET)\end{tabular}            & \begin{tabular}[c]{@{}l@{}}CORESET is a set of physical resources and a set of \\ parameters that is used to carry  PDCCH/DCI.\end{tabular}                                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Physical Downlink \\ Shared Channel (PDSCH)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}PDSCH is a downlink physical channel that \\ delivers user data from gNB to UE.\end{tabular}                                                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Physical Uplink \\ Share Channel (PUSCH)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}PUSCH is a uplink physical channel that delivers \\ user data from UE to gNB.\end{tabular}                                                                        \\ \hline
% \begin{tabular}[c]{@{}l@{}}Random Access \\ Channel (RACH)\end{tabular}              & \begin{tabular}[c]{@{}l@{}}RACH is the first channel used by UE to access \\ 5G service in UL.\end{tabular}                                                                                  \\ \hline
% Bandwidth Part (BWP)                                                                 & \begin{tabular}[c]{@{}l@{}}Base station in 5G split the whole frequency band into \\ multiple BWPs, the RACH process and later data\\ communication are conducted in different BWPs.\end{tabular} \\ \hline
% \end{tabular}
% \end{tiny}
% \caption{Physical Channel Definitions}
% \label{tab:physical_channel}
% \end{table}

% \begin{table}[]
% \begin{tiny}
% \begin{tabular}{l|l}
% \hline
% \multicolumn{1}{c|}{Terms (Acronym)}                                          & \multicolumn{1}{c}{Definition}                                                                                                                                                                                                                                                                    \\ \hline
% \begin{tabular}[c]{@{}l@{}}Radio Resource \\ Control (RRC)\end{tabular}       & \begin{tabular}[c]{@{}l@{}}RRC is a layer 3 (Network Layer) protocol used between UE and \\ Base Station. The major functions of the RRC protocol include \\ connection establishment and release functions, broadcast of \\ system information, and \textit{etc.}\end{tabular}  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Master Information \\ Block (MIB)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}A data block that carries the essential information about the radio \\ bearer, physical channel, and transport channel of the 5G RAN.\end{tabular}                                                                                                                     \\ \hline
% \begin{tabular}[c]{@{}l@{}}System Information \\ Blocks (SIBs)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}SIBs are broadcasted information blocks that contain system info-\\ rmation elements, including physical channel configuration and \textit{etc.}\end{tabular}                                                                                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}Preamble Transmission\\ (PRACH/MSG 1)\end{tabular} & \begin{tabular}[c]{@{}l@{}}The UE selects and sends random access preamble from a set of\\ predefined preambles, through which both sides agree on RA-RNTI.\end{tabular}                                                                                                                          \\ \hline
% \begin{tabular}[c]{@{}l@{}}Random Access \\ Response (RAR/MSG 2)\end{tabular} & \begin{tabular}[c]{@{}l@{}}After receiving MSG 1, gNB sends the RAR to UE using RA-RNTI, \\ which carries information, such as Time Advance for UE to adjust \\ its sending buffer and TC-RNTI.\end{tabular}                                                                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}RRC Setup \\ Request (MSG 3)\end{tabular}          & \begin{tabular}[c]{@{}l@{}}The UE sends a connection request message using the resources\\ granted in the RAR. This message contains the UE’s identity and \\ the reason for the establishment (e.g., initial access, handover, etc.).\end{tabular}                                               \\ \hline
% RRC Setup (MSG 4)                                                             & \begin{tabular}[c]{@{}l@{}}The gNB sends MSG 4 to UE and tells the UE more information\\ about the cell, such as the masterCellGroup in the Appendix~\ref{appd:msg4}. \\ After the message, the UE is RRC connected and initiates the \\ Registration process.\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Downlink Control \\ Information (DCI)\end{tabular} & \begin{tabular}[c]{@{}l@{}}DCI is the physical layer control information sent from the \\ gNB to the UE in each TTI and informs the UE the resource \\ blocks it should receive data from or send data to.\end{tabular}                                                                           \\ \hline
% \end{tabular}
% \caption{Radio Resource Control messages and Downlink Control Information.}
% \label{tab:rrc}
% \end{tiny}
% \end{table}

% \begin{table}[]
% \begin{tiny}
% \begin{tabular}{l|l}
% \hline
% % \multicolumn{1}{c|}{Terms (Acronym)}                                         & \multicolumn{1}{c}{Definition}                                                                                                                                                                                          \\ \hline
% \begin{tabular}[c]{@{}l@{}}System Information \\ RNTI (SI-RNTI)\end{tabular} & \begin{tabular}[c]{@{}l@{}}The UE uses SI-RNTI to receive SIBs during the initial \\ access procedure in 5G NR. It's always 0xFFFF.\end{tabular}                                                                        \\ \hline
% \begin{tabular}[c]{@{}l@{}}Random Access \\ RNTI (RA-RNTI)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}After the UE sends the MSG 1, both the UE and the gNB \\ can calculate RA-RNTI based on the parameters of the \\ preambles, through which thhe gNB sends MSG 2.\end{tabular}                 \\ \hline
% \begin{tabular}[c]{@{}l@{}}Temporal Cell \\ RNTI (TC-RNTI)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}The UE receives the MSG 2 with RA-RNTI and the it \\ decodes the TC-RNTI from the MSG 2, then it uses the \\ resources allocated in MSG 2 and uses TC-RNTI to \\ receive MSG 4.\end{tabular} \\ \hline
% Cell RNTI (C-RNTI)                                                           & \begin{tabular}[c]{@{}l@{}}After the RACH process, the UE promotes TC-RNTI to\\ C-RNTI and uses it as its identifier for all the data \\ communication afterward.\end{tabular}                                          \\ \hline
% \end{tabular}
% \caption{Radio Network Temporary Identifiers.}
% \label{tab:rnti}
% \end{tiny}
% \end{table}

==> sections/background.tex <==
% \subsection{Cloud Gaming and RTSP}
% %
% RTSP is an application layer protocol for multiplexing and packetizing multimedia transport streams.
% %
% RTSP is widely used in gaming platform to setup gaming streams, including downlnk video, audio streams and uplink control, microphone stream.
% %
% Mobile client and the gaming platform perform the handshake and agree on different streams' protocol type, port and \textit{etc.}, through RTSP standard messages, including $OPTION$, $DESCRIBE$, $SETUP$, $ANNOUNCE$ and \textit{etc.}~\cite{rtsp-org}. 
% %
% The actual streams can be transmitted through either TCP or UDP transport layer protocol and UDP is favored in gaming platform for low latency.
